Obstacle-Aware Four-Dimensional Trajectory Design for Urban Air Mobility

Urban Air Mobility (UAM) with electric Vertical TakeOff and Landing (eVTOL) vehicles can help address ground traffic congestion. The design of an eVTOL trajectory that is safe and reduces travel time is key for UAM adoption. Existing works on trajectory design either may not adequately incorporate dense obstacles in urban environments, complex eVTOL flight dynamics, or one or more flight phases. Not considering these factors can result in low-quality, or worse infeasible, trajectories. We develop a hybrid framework that can integrate building obstacles data, wind data, eVTOL flight dynamics, and other real-world operational constraints to estimate a four-dimensional eVTOL flight trajectory in ascent, cruise, and descent that aims to minimize travel time. Our framework first fills the obstacle-free regions with intersecting convex polygons, then identifies potentially low-travel time candidate sequences of these polygons using a Graph of Convex Sets-based path planner, and then uses an Optimal Control Program to give the final trajectory that passes through the polygons in a sequence identified before. We evaluate our framework on routes within New York City. Our framework can design trajectories respecting the above constraints in the presence of as many as 250 building obstacles. We show that not including the above constraints can underestimate the flight time by as much as 20\%.

==> 4_Nomenclature.tex <==
\begin{table}[btp]
	\caption{Nomenclature, bounds, and OCP initial guess values for different variables (`As': ascent phase; `Cr': cruise phase; `De': descent phase; `NA': Not Applicable. $D_\textrm{init} = 0.5\rho (W_N^2 + W_E^2 + 1.5^2)\mathcal{S}C_D$) 
		%		$h_s = \max(h_0+L, h_\textrm{min}, h_F+L)$. $D_\textrm{init} = 0.5\rho (W_N^2 + W_E^2 + {V_v}_\textrm{max}^2)\mathcal{S}C_D$
	}
	\label{Tab: nomenclature}
	\centering
	\begin{tabular}{|p{1cm}||p{0.7cm}||p{0.5cm}||p{1.6cm}||p{2.4cm}|}
		\hline
		\textbf{Variable} & \textbf{Sym./} & \textbf{Phase} &  \textbf{Value/Bounds} & \textbf{Initial Guess}\\
		& \textbf{Unit} & & & \\
		\hline
		
		\multirow{3}{*}{Latitude} & \multirow{3}{*}{$\lambda$,} & As & $\lambda_0$ & NA \\
		& \multirow{3}{*}{rad} & Cr & $[-\pi/2, \pi/2]$ & Refer Sec. \ref{Subsec: transcription} \\
		& & De & $\lambda_F$ & NA \\ %\hline
		
		\multirow{3}{*}{Longitude} & \multirow{3}{*}{$\tau$, } & As & $\tau_0$ & NA \\
		& \multirow{3}{*}{rad} & Cr & $[-\pi, \pi]$ & Refer Sec. \ref{Subsec: transcription}\\
		& & De & $\tau_F$ & NA \\ %\hline
		
		\multirow{3}{*}{Altitude} & \multirow{3}{*}{$h$, } & As &  $[h_0, h_c]$ & $\{h_0+i\frac{h_c-h_0}{N_\textrm{as}}|i = 0 \textrm{ to } N_\textrm{as}\}$\\
		& \multirow{3}{*}{m} & Cr & $h_c$ & $h_c$\\
		& & De & $[h_c, h_F]$ & $\{h_c+i\frac{h_F-h_c}{N_\textrm{de}}|i = 0 \textrm{ to } N_\textrm{de}\}$\\ %\hline
		
		Minimum cruising altitude & $h_\mathrm{min}$, m AMSL & Cr & max(135, $h_0 + L_v$, $h_F + L_v$) & NA\\ %\hline
		
		Maximum cruising altitude & $h_\mathrm{max}$, m AMSL & Cr & 1,225 & NA\\ %\hline

		
		Time/ & \multirow{3}{*}{$t$, } & As &  $\ge 0$ & $\frac{h_c-h_0}{1.5}$\\
		Travel & \multirow{3}{*}{s} & Cr & $\ge 0$ & Refer Sec. \ref{Subsec: transcription}\\
		duration & & De & $\ge 0$ & $\frac{h_c-h_F}{1.5}$\\ %\hline
		
		Northward & $W_N$, & All & 4.9 & NA \\
		wind & ms$^{-1}$ & & & \\ %\hline
		
		Eastward & $W_E$, & All & 1.6 & NA \\
		wind & ms$^{-1}$ & & & \\ %\hline
		
		\multirow{3}{*}{Horizontal} & \multirow{3}{*}{$V_l$, } & As &  $\sqrt{W_N^2 + W_E^2}$ & NA \\
		\multirow{3}{*}{airspeed}& \multirow{3}{*}{ms$^{-1}$} & Cr & $[0, 50.4]$ & 50.4 \\
		& & De & $\sqrt{W_N^2 + W_E^2}$ & NA \\ %\hline
		
		\multirow{3}{*}{Vertical} & \multirow{3}{*}{$V_v$, } & As &  $[0, 1.5]$ & 1.5 \\
		\multirow{3}{*}{airspeed}& \multirow{3}{*}{ms$^{-1}$} & Cr & 0 & NA \\
		& & De & $[-1.5, 0]$ & -1.5 \\ %\hline	
		
		\multirow{3}{*}{Thrust} & \multirow{3}{*}{$T$, } & As &  $\ge 0$ & $mg + D_\textrm{init}$\\
		& \multirow{3}{*}{N} & Cr & $\ge 0$ & NA\\
		& & De & $\ge 0$ & $|mg -  D_\textrm{init}|$\\ %\hline
		
		\multirow{3}{*}{Rotor} & \multirow{3}{*}{$\theta$, } & As &  $[-\pi/6, \pi/6]$ & $\tan^{-1}(\frac{ D_\textrm{init}}{mg})$\\
		\multirow{3}{*}{pitch} & \multirow{3}{*}{rad} & Cr & $[-\pi/6, \pi/6]$ & 0.1\\
		& & De & $[-\pi/6, \pi/6]$ & $\tan^{-1}(\frac{ D_\textrm{init}}{mg})$\\ %\hline
		
		\multirow{3}{*}{Rotor} & \multirow{3}{*}{$\dot{\theta}$, } & As &  $[-\pi/18, \pi/18]$ & NA\\
		\multirow{3}{*}{pitch rate} & \multirow{3}{*}{rad/s} & Cr & $[-\pi/18, \pi/18]$ & NA\\
		& & De & $[-\pi/18, \pi/18]$ & NA\\ %\hline
		
		Rotor angle of attack & $\alpha$ & All & $[-\pi/2, \pi/2]$ & NA\\ %\hline
		
		\multirow{3}{*}{Roll} & \multirow{3}{*}{$\phi$, } & As &  0 & NA \\
		& \multirow{3}{*}{rad} & Cr & $[-\pi/6, \pi/6]$ & 0.1\\
		& & De & 0 & NA \\ %\hline
		
		\multirow{3}{*}{Roll} & \multirow{3}{*}{$\dot{\phi}$, } & As &  $[-\pi/18, \pi/18]$ & NA\\
		\multirow{3}{*}{rate} & \multirow{3}{*}{rad/s} & Cr & $[-\pi/18, \pi/18]$ & NA\\
		& & De & $[-\pi/18, \pi/18]$ & NA\\ %\hline
		
		\multirow{3}{*}{Heading} & \multirow{3}{*}{$\psi$, } & As &  $\tan^{-1}(\frac{-W_E}{-W_N})$ & NA\\
		& \multirow{3}{*}{rad} & Cr & $[-\pi, \pi]$ & Great circle bearing\\
		& & De & $\tan^{-1}(\frac{-W_E}{-W_N})$ & NA \\ %\hline
		
%		\multirow{3}{*}{Flight} & \multirow{3}{*}{$\gamma$, } & As &  $[-\pi/2, \pi/2]$ & NA\\
%		\multirow{3}{*}{path angle} & \multirow{3}{*}{rad} & Cr & 0 & NA\\
%		& & De & $[-\pi/2, \pi/2]$ & NA\\ %\hline
		
		Required power & $P$, W & All & $\le$ 494,250 & NA\\ %\hline
		
		%Air density & $\rho$, $\mathrm{kgm^{-3}}$ & All & 1.225  & NA\\ \hline
		
		Vehicle mass & $m$, kg & All & 2,940 & NA\\ %\hline
		
		Vehicle ref. area & $\mathcal{S}$, m$^2$ & All & 1.1984 & NA\\ %\hline

		Vehicle drag coefficient & $C_D$ & All & 1 & NA\\ %\hline
				
		%Acc. due to gravity & $g$, $\mathrm{ms^{-2}}$ & All & 9.8 & NA\\ \hline
		
		%Earth radius & $R_e$, m & All & 6,371,000 & NA\\ \hline

		Lateral safety buffer & $L_l$, m & Cr & 25 & NA \\	
		
		Vertical safety buffer & $L_v$, m & Cr & 50 & NA \\
		\hline 
		
	\end{tabular}	
\end{table}


==> 5_GCS_OCP.tex <==
\section{Hybrid Framework for Trajectory Design} \label{Sec: GCS OCP}
To overcome the problem of convergence resulting from the feasible obstacle-free region being non-convex, we make a change in the obstacle avoidance constraint formulation. Instead of constraining the cruise trajectory to avoid obstacles, we constrain it to pass through intersecting convex polygons that make up the feasible region. We describe a new hybrid framework called `GCS-OCP' for trajectory design in Algorithm \ref{Alg}. The algorithm starts with a prescribed trajectory start point $s = (\lambda_0, \tau_0, h_0)$ at the origin vertiport, a prescribed goal point $g = (\lambda_F, \tau_F, h_F)$ at the destination vertiport, and a prescribed cruising altitude $h_c$. It also takes in as inputs various datasets and parameters.
We assume some example values of the parameters just for demonstration in this paper. The different modules of the algorithm are as follows: \input{5_algorithm}

\begin{enumerate}
\item \textproc{CreateGrid} (Line~\ref{Alg: grid} in Algorithm \ref{Alg}): Similar to Fig. 3 in \cite{Chati2025}, we first generate a two dimensional horizontal grid of $J$ seed points (denoted by $\mathbf{p}$), which are along and perpendicular to the straight line (great circle) path from the start of cruise (with coordinates $(\lambda_0, \tau_0, h_c)$; denoted by $p_0$) to the end of cruise with coordinates $(\lambda_F, \tau_F, h_c)$; denoted by $p_{J}$). This cruise grid plane is also perpendicular to the vertical ascent and descent phases. \textcolor{red}{Each point is at most 200 m away from its immediate neighbor.} The grid extends to a variable width $\Delta \in [500, 1500]$ m on either side of the straight line path over which we iterate. The obstacles appear as two-dimensional polygons in this cruise grid plane (when viewed from above). We reject any seed point which lies within with an obstacle. We enforce $p_0$ and $p_J$ to also be seed points. We conduct all analyses in the
NYC-specific NAD83 Cartesian coordinate system.

\item \textproc{GetObstacles} (Line~\ref{Alg: obstacles} in Algorithm \ref{Alg}): We use the input dataset (BD) on buildings (with polygonal planforms) to get the set of $n_o$ obstacles $\mathcal{O}$ in cruise. As mentioned in Sec. \ref{Subsec: obstacles direct OCP}, we include only those buildings whose height plus the safety buffer $L$ exceeds $h_c$. We also apply $L$ laterally around each such building. We retain only those obstacles in $\mathcal{O}$ whose buffered planform polygons intersect the rectangular grid of seed points defined above. We directly use the buffered planform polygons as obstacles and, unlike D-OCP, do not convert them to circular obstacles. In this paper, we assume $L$ = 50 m. 

\item \textproc{GetConvexSafeRegions} (Line~\ref{Alg: IRIS} in Algorithm \ref{Alg}): We use the Iterative Regional Inflation by Semi-definite programming (IRIS) algorithm \cite{Deits2014} to deconstruct the obstacle-free safe region into intersecting convex polygons. For each seed point, the IRIS algorithm starts by creating an initial ellipse which is tiny circle centered at the seed point. Next, it iterates through the obstacles and constructs a tangent to each obstacle polygon that separates the obstacle from the ellipse. The intersection of the set of such tangents for all the obstacles and the sides of the grid bounding rectangle gives a convex polygon enclosing the ellipse and separating it from the obstacles. Next, the algorithm finds a new maximal ellipse in the convex polygon given by the intersecting tangents. This alternation between constructing an ellipse and finding the set of tangents that result in a convex polygon enclosing the ellipse continues till the ellipse's rate of growth falls below some threshold. On converging, the algorithm returns the final obstacle-free convex polygon and the enclosed ellipsoid for each seed point. Running the IRIS algorithm for all the seed points results in a decomposition of the safe region into $n_p$ intersecting convex polygons $\mathcal{P}$. We discard any polygon that completely lies within or is a near duplicate of another polygon in a post-processing pruning step. 

Each such convex polygon, which is the intersection of $\zeta_i$ separating tangents and the sides of the grid bounding rectangle, can be mathematically represented as $\mathcal{P}_i := \{\mathbf{x}|\mathbf{A}_i\mathbf{x} \le \mathbf{b}_i\}$, where $\mathbf{x} \in \mathbb{R}^2, \mathbf{A_i} \in \mathbb{R}^{\zeta_i \times 2}, \textrm{and } \mathbf{b_i} \in \mathbb{R}^{\zeta_i}$. 
We refer the reader to \cite{Deits2014} for the mathematical details of the optimization problem that is solved in the IRIS algorithm. \textcolor{red}{Should we add here?}

%The ellipse is defined as the image of a unit circle: $\mathcal{E}(\mathbf{C}, \mathbf{d)} := \{\mathbf{x} = \mathbf{C}{\mathbf{\tilde{x}} + \mathbf{d}| \hspace{0.1cm} ||\mathbf{\tilde{x}}||_2 \le 1\}$, where in the two-dimensional cruise grid plane, $\mathbf{x, \tilde{x}} \in \mathbb{R}^2, \mathbf{C} \in \mathbb{R}^{2 \times 2}, \mathbf{d} \in \mathbb{R}^2$. The set of all $n_\zeta$ separating tangents is defined as $\zeta := \{\mathbf{x}|\mathbf{Ax} \le \mathbf{b}\}$, where $\mathbf{A} \in \mathbb{R}^{n_\zeta \times 2}, \mathbf{b} \in \mathbb{R}^{n_\zeta}$. 
	
\item \textproc{CreateGcs} (Line~\ref{Alg: GCS graph} in Algorithm \ref{Alg}): We create a bidirectional Graph of Convex Sets (GCS) $\mathcal{G} := (\mathcal{V}, \mathcal{E})$. Each convex polygon $\mathcal{P}_i$ given by the IRIS algorithm in the safe region is a vertex $\nu \in \mathcal{V}$ of the graph. We create an edge $e_{ij} \in \mathcal{E}$ from vertex $\nu_i$ to vertex $\nu_j$ if polygon $\mathcal{P}_i$ intersects with polygon $\mathcal{P}_j$. Each such edge $e$ (where we henceforth, ignore the subscript $ij$ for ease of notation) has a starting point $\mathbf{x}_e \in \mathcal{P}_i$, an end point $\mathbf{x}'_{e} \in \mathcal{P}_j$, and an edge weight $w_{e} := \frac{||\mathbf{x}'_e - \mathbf{x}_e||_2}{V_{g_{ij}}}$ which is the time taken to traverse the edge from $\mathbf{x}_e$ to $\mathbf{x}'_e$. This time is given by the length of the edge divided by the eVTOL ground speed $V_g$ along the directed edge. We estimate this ground speed by applying the parallelogram law of vector addition to the maximum horizontal airspeed ($\overrightarrow{V_\textrm{l, max}}$) and the wind velocity ($\overrightarrow{W}$) vectors in cruise ($\overrightarrow{V_g} = \overrightarrow{V_\textrm{l, max}} + \overrightarrow{W}$).

\item \textproc{GetCandidatePaths} (Line~\ref{Alg: GCS path} in Algorithm \ref{Alg}): Once the graph $\mathcal{G}$ is constructed, we aim to get time-optimal paths (i.e., sequence of convex polygons $\mathcal{P}_i$) from the convex polygon (i.e., graph vertex) containing the cruise start point $p_0$ to that containing the cruise end point $p_J$ using a GCS-based planner. First, with each edge $e$ we associate two variables: i) a flow variable $y_{e} \in \{0, 1\}$ which indicates if the edge is a part of the path or not, and ii) a variable $\beta_e \ge 0$ that we will use in the optimization objective function. Second, we also define two auxiliary variables $\mathbf{z}_e := \mathbf{x}_ey_{e}$ and $\mathbf{z}'_e := \mathbf{x}'_ey_{e}$. Then the path can be given as the solution of the following mixed-integer convex program (MICP) (\cite{Marcucci2024}):

\begin{align}
	\nonumber
	\textrm{minimize} \sum_{e \in \mathcal{E}}\beta_e && \\
	\nonumber
	\textrm{subject to: } V_{g, \textrm{max}}\beta_e \ge ||\mathbf{z}'_e - \mathbf{z}_e||_2 \hspace{0.5cm} \forall e \in \mathcal{E}; \\
	\nonumber
	\sum_{e \in \mathcal{E}_{p_0}^{\textrm{out}}}y_{e} = 1; 
	\sum_{e \in \mathcal{E}_{p_J}^{\textrm{in}}}y_{e} = 1; \\
	\nonumber
	\sum_{e \in \mathcal{E}_{\nu}^{\textrm{out}}}y_{e} \le 1 \hspace{0.5cm} \forall \nu \in \mathcal{V} - \{p_0, p_J\}; \\
	\nonumber
	\sum_{e \in \mathcal{E}_{\nu}^{\textrm{out}}}y_{e} = \sum_{e \in \mathcal{E}_{\nu}^{\textrm{in}}}y_{e} \hspace{0.5cm} \forall \nu \in \mathcal{V} - \{p_0, p_J\}; \\
	\nonumber
	\sum_{e \in \mathcal{E}_{\nu}^{\textrm{out}}}y_{e} = \sum_{e \in \mathcal{E}_{\nu}^{\textrm{in}}}y_{e} \hspace{0.5cm} \forall \nu \in \mathcal{V} - \{p_0, p_J\}; \\
	\nonumber
	\sum_{e \in \mathcal{E}_{\nu}^{\textrm{out}}}\mathbf{z}_{e} = \sum_{e \in \mathcal{E}_{\nu}^{\textrm{in}}}\mathbf{z}'_{e} \hspace{0.5cm} \forall \nu \in \mathcal{V} - \{p_0, p_J\}; \\
	\nonumber
	\mathbf{A}_i\mathbf{z}_e \le \mathbf{b}_iy_e, \hspace{0.1cm} \mathbf{A}_j\mathbf{z}'_e \le \mathbf{b}_jy_e \hspace{0.5cm} \forall e_{ij} \in \mathcal{E}; \\
	y_e \in \{0, 1\} \hspace{0.5cm} \forall e \in \mathcal{E} \label{Eq: GCS formulation}
\end{align}
where, $V_{g, \textrm{max}}$ is an upper bound on the possible ground speed. To reduce the computational cost of this MICP, we resort to a convex relaxation whereby instead of constraining $y_e$ to be a binary variable $y_e \in \{0, 1\}$, we relax it to be a real variable $y_e \in [0, 1]$. This relaxation is tight in practice and almost always sufficient to design an optimal trajectory \cite{Marcucci2023}. Instead of using an exact branch-and-bound solution technique, we solve this convex relaxation fast and get an approximate solution for the different variables involved.

Based on the above solution, to get a candidate time-optimal path (i.e., sequence of convex flight-safe polygons) $\epsilon$, we start at vertex $p_0$. We choose the next edge with a probability proportional to the solved value of its flow variable $y_e$. We continue this process till we reach the end vertex $p_J$, all the while ensuring that no vertex is visited twice. Performing this cheap randomized rounding technique multiple times gives us many candidate paths that can potentially give time-optimal cruise trajectories. We also consider candidate paths where the edges having the maximum value of the flow variable are chosen greedily. We order all these candidate paths by their total travel time given as the sum of the weights $w_e$ for all the edges in a path. We retain only the top few candidate paths to get the set $\mathcal{C}$ of good candidate paths $\epsilon$. We refer the reader to \cite{Marcucci2024, Marcucci2023} for more details of the GCS-based planner.

\item \textproc{RunOcp} (Line~\ref{Alg: GCS-OCP} in Algorithm \ref{Alg}): We run an OCP to get the final time-optimal trajectory. We use the same variables, performance index, path constraints, and boundary constraints as described in Sec. \ref{Sec: framework}. However, this OCP differs from the direct OCP (D-OCP) in the manner the obstacle avoidance constraint is formulated in cruise. We divide the cruise trajectory into multiple parts and map each part, in order, to a convex polygon in one candidate path $\epsilon_i$ found above. For part $c_i$ mapped to polygon $\mathcal{P}_i$, we enforce the cruise trajectory in part $c_i$ to lie wholly within polygon $\mathcal{P}_i$, that is $\mathbf{A}_i\mathbf{x} \le \mathbf{b}_i$
for each point $\mathbf{x}$ on the cruise trajectory in part $c_i$. Here, $\mathbf{x}$ is the NAD83 Cartesian projection of a cruise trajectory point with coordinates $(\lambda, \tau)$.

\item \textproc{GetOptimalTrajectory} (Line~\ref{Alg: optimal solution} in Algorithm \ref{Alg}): Running the OCP for each candidate path $\epsilon \in \mathcal{C}$ gives us a set of trajectories and times of flight $\{\mathrm{Traj}(\epsilon), t_F(\epsilon)|\epsilon \in \mathcal{C}\}$. From this set, we choose the final time-optimal trajectory (denoted by `Traj$^*$') as the one with the shortest time of travel (denoted by $t_F^*$). 
\end{enumerate}

%\item \textproc{GetBestTrajectory} (Line~\ref{Alg: best altitude} in Algorithm \ref{Alg}): For the prescribed start and end points, the best cruising altitude $h_c^\textrm{best}$ is the altitude that gives the lowest $t_F^*$ among all the altitudes for which we have obtained the trajectories above. We denote by `Traj$_\textrm{best}$' and $t_{F, \textrm{best}}$ the best trajectory and travel time over all the altitudes.


